occ2vec: A principal approach to representing occupations using natural language processing

We propose \textbf{occ2vec}, a principal approach to representing occupations, which can be used in matching, predictive and causal modeling, and other economic areas. In particular, we use it to score occupations on any definable characteristic of interest, say the degree of \textquote{greenness}. Using more than 17,000 occupation-specific text descriptors, we transform each occupation into a high-dimensional vector using natural language processing. Similar, we assign a vector to the target characteristic and estimate the occupational degree of this characteristic as the cosine similarity between the vectors. The main advantages of this approach are its universal applicability and verifiability contrary to existing ad-hoc approaches. We extensively validate our approach on several exercises and then use it to estimate the occupational degree of charisma and emotional intelligence (EQ). We find that occupations that score high on these tend to have higher educational requirements. Turning to wages, highly charismatic occupations are either found in the lower or upper tail in the wage distribution. This is not found for EQ, where higher levels of EQ are generally correlated with higher wages.

==> tables/assessment/listings_topbottom10_concept_age_friendliness.tex <==
\begin{tabular}{lll}
\toprule
{} &                                             Top 10 &                                          Bottom 10 \\
Rank &                                                    &                                                    \\
\midrule
1    &     Equal Opportunity Representatives and Officers &  Outdoor Power Equipment and Other Small Engine... \\
2    &                 Compensation and Benefits Managers &     Electrical Power-Line Installers and Repairers \\
3    &                      Proofreaders and Copy Markers &   Mobile Heavy Equipment Mechanics, Except Engines \\
4    &                                New Accounts Clerks &                              Helpers--Electricians \\
5    &                         Treasurers and Controllers &                               Motorcycle Mechanics \\
6    &                           Mental Health Counselors &                               Robotics Technicians \\
7    &                            Recreational Therapists &                          Hoist and Winch Operators \\
8    &                           Self-Enrichment Teachers &                                       Electricians \\
9    &  Human Resources Assistants, Except Payroll and... &  Electric Motor, Power Tool, and Related Repairers \\
10   &                       Health Education Specialists &  Bus and Truck Mechanics and Diesel Engine Spec... \\
\bottomrule
\end{tabular}


==> tables/assessment/listings_topbottom10_concept_cognitive_ability.tex <==
\begin{tabular}{lll}
\toprule
{} &                                             Top 10 &                                          Bottom 10 \\
Rank &                                                    &                                                    \\
\midrule
1    &                               School Psychologists &                          Mechanical Door Repairers \\
2    &              Poets, Lyricists and Creative Writers &                                            Riggers \\
3    &                                     Mathematicians &                     Derrick Operators, Oil and Gas \\
4    &                                   Online Merchants &                                  Bicycle Repairers \\
5    &                       Speech-Language Pathologists &                     Maintenance Workers, Machinery \\
6    &                             Office Clerks, General &              Fiberglass Laminators and Fabricators \\
7    &              Special Education Teachers, Preschool &                               Roof Bolters, Mining \\
8    &           Credit Authorizers, Checkers, and Clerks &  Forging Machine Setters, Operators, and Tender... \\
9    &  Low Vision Therapists, Orientation and Mobilit... &  Outdoor Power Equipment and Other Small Engine... \\
10   &                              Intelligence Analysts &           Structural Metal Fabricators and Fitters \\
\bottomrule
\end{tabular}


==> tables/assessment/listings_topbottom10_concept_crystallized_intelligence.tex <==
\begin{tabular}{lll}
\toprule
{} &                                             Top 10 &                                          Bottom 10 \\
Rank &                                                    &                                                    \\
\midrule
1    &                                         Historians &  Extruding and Drawing Machine Setters, Operato... \\
2    &                  Anthropologists and Archeologists &  Cutting and Slicing Machine Setters, Operators... \\
3    &                              Intelligence Analysts &  Cutting, Punching, and Press Machine Setters, ... \\
4    &                     Business Intelligence Analysts &  Extruding, Forming, Pressing, and Compacting M... \\
5    &                       Search Marketing Strategists &  Woodworking Machine Setters, Operators, and Te... \\
6    &           Credit Authorizers, Checkers, and Clerks &  Milling and Planing Machine Setters, Operators... \\
7    &  Human Resources Assistants, Except Payroll and... &          Automotive Glass Installers and Repairers \\
8    &                                        Geographers &  Multiple Machine Tool Setters, Operators, and ... \\
9    &        Court Reporters and Simultaneous Captioners &  Rolling Machine Setters, Operators, and Tender... \\
10   &  Market Research Analysts and Marketing Special... &     Glass Blowers, Molders, Benders, and Finishers \\
\bottomrule
\end{tabular}


==> tables/assessment/listings_topbottom10_concept_fluid_intelligence.tex <==
\begin{tabular}{lll}
\toprule
{} &                                        Top 10 &                                          Bottom 10 \\
Rank &                                               &                                                    \\
\midrule
1    &                                Mathematicians &                                            Barbers \\
2    &                                 Statisticians &  Rolling Machine Setters, Operators, and Tender... \\
3    &                                    Physicists &                        Floor Sanders and Finishers \\
4    &                                   Geographers &  Helpers--Brickmasons, Blockmasons, Stonemasons... \\
5    &                  Forensic Science Technicians &                 Shoe Machine Operators and Tenders \\
6    &                                   Astronomers &     Hairdressers, Hairstylists, and Cosmetologists \\
7    &                         Intelligence Analysts &                     Terrazzo Workers and Finishers \\
8    &  Computer and Information Research Scientists &                               Skincare Specialists \\
9    &                              Biostatisticians &                                         Shampooers \\
10   &   Remote Sensing Scientists and Technologists &                 Solar Energy Installation Managers \\
\bottomrule
\end{tabular}


==> tables/assessment/listings_topbottom10_concept_job_training.tex <==
\begin{tabular}{lll}
\toprule
{} &                                             Top 10 &                                        Bottom 10 \\
Rank &                                                    &                                                  \\
\midrule
1    &               Training and Development Specialists &                                 Biostatisticians \\
2    &                  Training and Development Managers &                                   Mathematicians \\
3    &    Exercise Trainers and Group Fitness Instructors &                     Operations Research Analysts \\
4    &             Adapted Physical Education Specialists &                                    Statisticians \\
5    &  Career/Technical Education Teachers, Postsecon... &                              Logistics Engineers \\
6    &                                    Animal Trainers &                            Wind Energy Engineers \\
7    &                             Exercise Physiologists &  Civil Engineering Technologists and Technicians \\
8    &  Adult Basic Education, Adult Secondary Educati... &                                       Physicists \\
9    &                      Physical Therapist Assistants &                            Industrial Ecologists \\
10   &                           Self-Enrichment Teachers &                               Procurement Clerks \\
\bottomrule
\end{tabular}


==> tables/assessment/listings_topbottom10_concept_meaningful_work.tex <==
\begin{tabular}{lll}
\toprule
{} &                                             Top 10 &                                          Bottom 10 \\
Rank &                                                    &                                                    \\
\midrule
1    &  Fine Artists, Including Painters, Sculptors, a... &  Plating Machine Setters, Operators, and Tender... \\
2    &                           Self-Enrichment Teachers &                        Floor Sanders and Finishers \\
3    &                Social Work Teachers, Postsecondary &  Outdoor Power Equipment and Other Small Engine... \\
4    &  Adult Basic Education, Adult Secondary Educati... &                          Counter and Rental Clerks \\
5    &              Poets, Lyricists and Creative Writers &  Separating, Filtering, Clarifying, Precipitati... \\
6    &                                             Clergy &  Coating, Painting, and Spraying Machine Setter... \\
7    &                       Search Marketing Strategists &                              Power Plant Operators \\
8    &                                            Nannies &                                Gas Plant Operators \\
9    &                 Teaching Assistants, Postsecondary &  Pesticide Handlers, Sprayers, and Applicators,... \\
10   &  Area, Ethnic, and Cultural Studies Teachers, P... &                              Endoscopy Technicians \\
\bottomrule
\end{tabular}


==> tables/assessment/listings_topbottom10_concept_paid_time_off.tex <==
\begin{tabular}{lll}
\toprule
{} &                                  Top 10 &                                          Bottom 10 \\
Rank &                                         &                                                    \\
\midrule
1    &  Adapted Physical Education Specialists &                                  Cytotechnologists \\
2    &                Physical Therapist Aides &                         Pourers and Casters, Metal \\
3    &              Occupational Therapy Aides &                             Microsystems Engineers \\
4    &                 Recreational Therapists &                            Gem and Diamond Workers \\
5    &           Physical Therapist Assistants &                   Quality Control Systems Managers \\
6    &         Occupational Therapy Assistants &                              Photonics Technicians \\
7    &          Payroll and Timekeeping Clerks &  Separating, Filtering, Clarifying, Precipitati... \\
8    &                  Exercise Physiologists &                                         Machinists \\
9    &                Self-Enrichment Teachers &                                Tool and Die Makers \\
10   &   Special Education Teachers, Preschool &                                           Chemists \\
\bottomrule
\end{tabular}


==> tables/assessment/listings_topbottom10_concept_physical_ability.tex <==
\begin{tabular}{lll}
\toprule
{} &                                             Top 10 &                                          Bottom 10 \\
Rank &                                                    &                                                    \\
\midrule
1    &             Adapted Physical Education Specialists &  Agents and Business Managers of Artists, Perfo... \\
2    &                             Exercise Physiologists &          Political Science Teachers, Postsecondary \\
3    &                    Athletes and Sports Competitors &                                      Tax Preparers \\
4    &    Exercise Trainers and Group Fitness Instructors &                                    Budget Analysts \\
5    &    Physical Medicine and Rehabilitation Physicians &                  Economics Teachers, Postsecondary \\
6    &                           Physical Therapist Aides &                     Business Intelligence Analysts \\
7    &                                            Dancers &    Philosophy and Religion Teachers, Postsecondary \\
8    &                      Physical Therapist Assistants &                Social Work Teachers, Postsecondary \\
9    &                              Construction Laborers &                        Law Teachers, Postsecondary \\
10   &  Laborers and Freight, Stock, and Material Move... &                                          Actuaries \\
\bottomrule
\end{tabular}


==> tables/assessment/listings_topbottom10_concept_physical_job_demands.tex <==
\begin{tabular}{lll}
\toprule
{} &                                           Top 10 &                                          Bottom 10 \\
Rank &                                                  &                                                    \\
\midrule
1    &                           Exercise Physiologists &  Agents and Business Managers of Artists, Perfo... \\
2    &           Adapted Physical Education Specialists &                              Wind Energy Engineers \\
3    &  Exercise Trainers and Group Fitness Instructors &                                    Budget Analysts \\
4    &                  Athletes and Sports Competitors &                     Business Intelligence Analysts \\
5    &  Physical Medicine and Rehabilitation Physicians &           Credit Authorizers, Checkers, and Clerks \\
6    &                         Physical Therapist Aides &  Compensation, Benefits, and Job Analysis Speci... \\
7    &                    Physical Therapist Assistants &                    Wind Energy Operations Managers \\
8    &                   Terrazzo Workers and Finishers &                                   Talent Directors \\
9    &                           Tile and Stone Setters &                                      Loan Officers \\
10   &           Painters, Construction and Maintenance &                 Compensation and Benefits Managers \\
\bottomrule
\end{tabular}


==> tables/assessment/listings_topbottom10_concept_power.tex <==
\begin{tabular}{lll}
\toprule
{} &                                             Top 10 &                                          Bottom 10 \\
Rank &                                                    &                                                    \\
\midrule
1    &           Arbitrators, Mediators, and Conciliators &                                  Bicycle Repairers \\
2    &                               Political Scientists &                        Floor Sanders and Finishers \\
3    &                               School Psychologists &                  Signal and Track Switch Repairers \\
4    &                           Investment Fund Managers &             Landscaping and Groundskeeping Workers \\
5    &                       Public Relations Specialists &       Meat, Poultry, and Fish Cutters and Trimmers \\
6    &  Administrative Law Judges, Adjudicators, and H... &              Automotive Body and Related Repairers \\
7    &      Directors, Religious Activities and Education &                          Tree Trimmers and Pruners \\
8    &                         Treasurers and Controllers &  Woodworking Machine Setters, Operators, and Te... \\
9    &         Judges, Magistrate Judges, and Magistrates &                          Sailors and Marine Oilers \\
10   &                                   Chief Executives &  Textile Cutting Machine Setters, Operators, an... \\
\bottomrule
\end{tabular}


==> tables/assessment/listings_topbottom10_concept_prestige.tex <==
\begin{tabular}{lll}
\toprule
{} &                                             Top 10 &                                          Bottom 10 \\
Rank &                                                    &                                                    \\
\midrule
1    &                    Athletes and Sports Competitors &  Pesticide Handlers, Sprayers, and Applicators,... \\
2    &                                     Choreographers &                                Traffic Technicians \\
3    &                                            Dancers &      Eligibility Interviewers, Government Programs \\
4    &                                             Models &                       Interpreters and Translators \\
5    &                           Cooks, Private Household &                           Agricultural Technicians \\
6    &                       Public Relations Specialists &                          Cytogenetic Technologists \\
7    &  Agents and Business Managers of Artists, Perfo... &                      Neurodiagnostic Technologists \\
8    &                     Terrazzo Workers and Finishers &                  Tank Car, Truck, and Ship Loaders \\
9    &                              Musicians and Singers &  Veterinary Assistants and Laboratory Animal Ca... \\
10   &                                     Range Managers &          Interviewers, Except Eligibility and Loan \\
\bottomrule
\end{tabular}


==> tables/assessment/listings_topbottom10_concept_schedule_flexibility.tex <==
\begin{tabular}{lll}
\toprule
{} &                                             Top 10 &                           Bottom 10 \\
Rank &                                                    &                                     \\
\midrule
1    &                             Exercise Physiologists &                        Hydrologists \\
2    &                  Fitness and Wellness Coordinators &        Forensic Science Technicians \\
3    &                     Payroll and Timekeeping Clerks &    Atmospheric and Space Scientists \\
4    &                    General and Operations Managers &           Bioinformatics Scientists \\
5    &            Meeting, Convention, and Event Planners &               Nanosystems Engineers \\
6    &             Adapted Physical Education Specialists &      Nuclear Medicine Technologists \\
7    &  Industrial Engineering Technologists and Techn... &           Soil and Plant Scientists \\
8    &                            Recreational Therapists &                   Cytotechnologists \\
9    &                                   Lodging Managers &          Bioinformatics Technicians \\
10   &                        Labor Relations Specialists &  Zoologists and Wildlife Biologists \\
\bottomrule
\end{tabular}


==> tables/assessment/listings_topbottom10_concept_teamwork.tex <==
\begin{tabular}{lll}
\toprule
{} &                                          Top 10 &                             Bottom 10 \\
Rank &                                                 &                                       \\
\midrule
1    &                                 Team Assemblers &                   Patternmakers, Wood \\
2    &                                    Sociologists &                   Furniture Finishers \\
3    &                 Athletes and Sports Competitors &                         Craft Artists \\
4    &                     Labor Relations Specialists &        Terrazzo Workers and Finishers \\
5    &                        Human Resources Managers &     Ophthalmic Laboratory Technicians \\
6    &            Training and Development Specialists &  Cement Masons and Concrete Finishers \\
7    &  Equal Opportunity Representatives and Officers &              Meter Readers, Utilities \\
8    &         Industrial-Organizational Psychologists &  Grinding and Polishing Workers, Hand \\
9    &   Umpires, Referees, and Other Sports Officials &                    Model Makers, Wood \\
10   &                                          Actors &           Floor Sanders and Finishers \\
\bottomrule
\end{tabular}


==> tables/assessment/listings_topbottom10_concept_telecommuting.tex <==
\begin{tabular}{lll}
\toprule
{} &                                             Top 10 &                                          Bottom 10 \\
Rank &                                                    &                                                    \\
\midrule
1    &                        Word Processors and Typists &                                        Podiatrists \\
2    &                             Office Clerks, General &               Grinding and Polishing Workers, Hand \\
3    &  Switchboard Operators, Including Answering Ser... &            Musical Instrument Repairers and Tuners \\
4    &                            Couriers and Messengers &                             Surgical Technologists \\
5    &    Legal Secretaries and Administrative Assistants &                                Tool and Die Makers \\
6    &                     Payroll and Timekeeping Clerks &                    Biofuels Processing Technicians \\
7    &  Secretaries and Administrative Assistants, Exc... &  Refractory Materials Repairers, Except Brickma... \\
8    &                              Postal Service Clerks &  Coating, Painting, and Spraying Machine Setter... \\
9    &                                Telephone Operators &  Outdoor Power Equipment and Other Small Engine... \\
10   &                                      Telemarketers &                  Ophthalmic Laboratory Technicians \\
\bottomrule
\end{tabular}


==> tables/assessment/listings_topbottom10_concept_work_autonomy.tex <==
\begin{tabular}{lll}
\toprule
{} &                                             Top 10 &                                          Bottom 10 \\
Rank &                                                    &                                                    \\
\midrule
1    &  Rail Yard Engineers, Dinkey Operators, and Hos... &                                     Mathematicians \\
2    &  Laborers and Freight, Stock, and Material Move... &                    Financial Quantitative Analysts \\
3    &                             Farm Labor Contractors &                         Sports Medicine Physicians \\
4    &                                    Team Assemblers &       Mathematical Science Teachers, Postsecondary \\
5    &  Welding, Soldering, and Brazing Machine Setter... &                                      Statisticians \\
6    &                     Machine Feeders and Offbearers &                                       Hydrologists \\
7    &                   Agricultural Equipment Operators &                     Business Intelligence Analysts \\
8    &    Dispatchers, Except Police, Fire, and Ambulance &                                          Actuaries \\
9    &  First-Line Supervisors of Production and Opera... &  Geographic Information Systems Technologists a... \\
10   &                                Personal Care Aides &                         Water Resource Specialists \\
\bottomrule
\end{tabular}


==> tables/assessment/listings_topbottom10_concept_work_pace.tex <==
\begin{tabular}{lll}
\toprule
{} &                                             Top 10 &                                   Bottom 10 \\
Rank &                                                    &                                             \\
\midrule
1    &                     Machine Feeders and Offbearers &                    Advertising Sales Agents \\
2    &  Rail-Track Laying and Maintenance Equipment Op... &   Solar Sales Representatives and Assessors \\
3    &                                             Tapers &                      Insurance Sales Agents \\
4    &                              Construction Laborers &                                    Curators \\
5    &  Industrial Engineering Technologists and Techn... &  Merchandise Displayers and Window Trimmers \\
6    &  Pressers, Textile, Garment, and Related Materials &                                      Clergy \\
7    &  Laborers and Freight, Stock, and Material Move... &                          Genetic Counselors \\
8    &        Production, Planning, and Expediting Clerks &                               Telemarketers \\
9    &                     Payroll and Timekeeping Clerks &                Search Marketing Strategists \\
10   &         Graders and Sorters, Agricultural Products &                                 Geneticists \\
\bottomrule
\end{tabular}


==> tables/comparison/comparing_ai_indices_correlation_method_kendall.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &  Brynjolfsson et al. (2018) &  Felten et al. (2018) &  Mühlbach (2022) &  Webb (2020) \\
\midrule
Brynjolfsson et al. (2018) &                       1.000 &                -0.061 &            0.190 &        0.039 \\
Felten et al. (2018)       &                      -0.061 &                 1.000 &            0.237 &        0.264 \\
Mühlbach (2022)            &                       0.190 &                 0.237 &            1.000 &        0.134 \\
Webb (2020)                &                       0.039 &                 0.264 &            0.134 &        1.000 \\
\bottomrule
\end{tabular}


==> tables/comparison/comparing_task_measure_indices_abstract_tasks_correlation_method_kendall.tex <==
\begin{tabular}{lrr}
\toprule
{} &  Autor et al. (2003) &  Mühlbach (2022) \\
\midrule
Autor et al. (2003) &                1.000 &            0.270 \\
Mühlbach (2022)     &                0.270 &            1.000 \\
\bottomrule
\end{tabular}


==> tables/comparison/comparing_task_measure_indices_abstract_tasks_correlation_method_spearman.tex <==
\begin{tabular}{lrr}
\toprule
{} &  Autor et al. (2003) &  Mühlbach (2022) \\
\midrule
Autor et al. (2003) &                1.000 &            0.401 \\
Mühlbach (2022)     &                0.401 &            1.000 \\
\bottomrule
\end{tabular}


==> tables/comparison/comparing_task_measure_indices_manual_tasks_correlation_method_kendall.tex <==
\begin{tabular}{lrr}
\toprule
{} &  Autor et al. (2003) &  Mühlbach (2022) \\
\midrule
Autor et al. (2003) &                1.000 &            0.631 \\
Mühlbach (2022)     &                0.631 &            1.000 \\
\bottomrule
\end{tabular}


==> tables/comparison/comparing_task_measure_indices_manual_tasks_correlation_method_spearman.tex <==
\begin{tabular}{lrr}
\toprule
{} &  Autor et al. (2003) &  Mühlbach (2022) \\
\midrule
Autor et al. (2003) &                1.000 &            0.835 \\
Mühlbach (2022)     &                0.835 &            1.000 \\
\bottomrule
\end{tabular}


==> tables/comparison/comparing_task_measure_indices_routine_tasks_correlation_method_kendall.tex <==
\begin{tabular}{lrr}
\toprule
{} &  Autor et al. (2003) &  Mühlbach (2022) \\
\midrule
Autor et al. (2003) &                1.000 &            0.446 \\
Mühlbach (2022)     &                0.446 &            1.000 \\
\bottomrule
\end{tabular}


==> tables/comparison/comparing_task_measure_indices_routine_tasks_correlation_method_spearman.tex <==
\begin{tabular}{lrr}
\toprule
{} &  Autor et al. (2003) &  Mühlbach (2022) \\
\midrule
Autor et al. (2003) &                1.000 &            0.635 \\
Mühlbach (2022)     &                0.635 &            1.000 \\
\bottomrule
\end{tabular}


==> tables/misc/assessment_R_estimation_lossnuc_testpct0_attrsplit0_33_reuseFalse.tex <==
\begin{tabular}{llrrrrrr}
\toprule
              &          & \multicolumn{3}{l}{Frobenius norm} & \multicolumn{3}{l}{Nuclear norm} \\
              &          &        average &   max &   min &      average &   max &   min \\
Sample & Strategy &                &       &       &              &       &       \\
\midrule
Full sample & IDENTITY &          1.000 & 1.000 & 1.000 &        1.000 & 1.000 & 1.000 \\
              & UR &          0.768 & 0.825 & 0.741 &        0.778 & 0.795 & 0.766 \\
              & DIAG &          0.894 & 0.935 & 0.852 &        1.004 & 1.008 & 0.998 \\
              & DIAG+NONNEG &          0.821 & 0.853 & 0.801 &        0.977 & 0.981 & 0.973 \\
              & DIAG+SUM &          0.915 & 0.971 & 0.862 &        1.023 & 1.033 & 1.016 \\
In-Sample & IDENTITY &          1.000 & 1.000 & 1.000 &        1.000 & 1.000 & 1.000 \\
              & UR &          0.000 & 0.000 & 0.000 &        0.000 & 0.000 & 0.000 \\
              & DIAG &          0.524 & 0.549 & 0.506 &        0.801 & 0.821 & 0.791 \\
              & DIAG+NONNEG &          0.609 & 0.642 & 0.571 &        0.865 & 0.884 & 0.845 \\
              & DIAG+SUM &          0.534 & 0.556 & 0.516 &        0.814 & 0.831 & 0.802 \\
Out-of-Sample & IDENTITY &          1.000 & 1.000 & 1.000 &        1.000 & 1.000 & 1.000 \\
              & UR &          0.921 & 0.949 & 0.859 &        1.044 & 1.036 & 1.029 \\
              & DIAG &          1.001 & 1.074 & 0.954 &        1.028 & 1.053 & 1.022 \\
              & DIAG+NONNEG &          0.909 & 0.957 & 0.862 &        0.989 & 1.013 & 0.993 \\
              & DIAG+SUM &          1.022 & 1.104 & 0.953 &        1.047 & 1.073 & 1.037 \\
\bottomrule
\end{tabular}


==> tables/misc/estimates_example.tex <==
\begin{tabular}{lcc}
\toprule 
 & Arbitrators & Roof Bolters\tabularnewline
\midrule
Oral Comprehension & 2.31 & -2.08\tabularnewline
Depth Perception & -1.95 & 2.13\tabularnewline
\bottomrule
\end{tabular}

==> tables/validation/validation_via_correlation_between_occupations_kendall.tex <==
\begin{tabular}{rrr}
\toprule
 $\rho=\rho_{0}$ &  $t$-stat &  $p$-value \\
\midrule
           0.000 &    35.818 &      0.000 \\
           0.390 &     1.228 &      0.221 \\
\bottomrule
\end{tabular}


==> tables/validation/validation_via_correlation_between_occupations_pearson.tex <==
\begin{tabular}{rrr}
\toprule
 $\rho=\rho_{0}$ &  $t$-stat &  $p$-value \\
\midrule
           0.000 &    39.569 &      0.000 \\
           0.540 &     1.731 &      0.085 \\
\bottomrule
\end{tabular}


==> tables/validation/validation_via_correlation_within_occupations_kendall.tex <==
\begin{tabular}{rrr}
\toprule
 $\rho=\rho_{0}$ &  $t$-stat &  $p$-value \\
\midrule
           0.000 &   210.202 &      0.000 \\
           0.580 &     0.773 &      0.440 \\
\bottomrule
\end{tabular}


==> tables/validation/validation_via_correlation_within_occupations_pearson.tex <==
\begin{tabular}{rrr}
\toprule
 $\rho=\rho_{0}$ &  $t$-stat &  $p$-value \\
\midrule
           0.000 &   287.809 &      0.000 \\
           0.770 &    -0.859 &      0.390 \\
\bottomrule
\end{tabular}

